Completing the Functional Approach in Object-Oriented Languages

Over the last two decades practically all object-oriented programming languages have introduced features that are well-known from functional programming languages. But many features that were introduced were fragmentary. In Java-TX we address the latter features and propose a completion. Java-TX (i.e. Type eXtended) is a language based on Java. The predominant new features are global type inference and real function types for lambda expressions. Global type inference means that all type annotations can be omitted, and the compiler infers them without losing the static type property. We introduce the function types in a similar fashion as in Scala but additionally integrated them into the Java target-typing as proposed in the so-called strawman approach. In this paper, we provide an integrated presentation of all Java-TX features. The focus is therby on the automatic inference of type parameters for classes and their methods, and on the heterogeneous translation of function types, which permits the preservation of the argument and return types in bytecode.

==> eptcsdata.tex <==
\providecommand{\firstpage}{43}
\providecommand{\publicationstatus}{Bieniusa, Degen, Wehr (Eds.). A Second Soul: \\
Celebrating the Many Languages of Programming\\
EPTCS 413, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.413.4}{10.4204/EPTCS.413.4}}
\pdfoutput=1

